An exact algorithm for the static pricing problem under discrete mixed logit demand

Price differentiation is a common strategy in many markets. In this paper, we study a static multiproduct price optimization problem with demand given by a discrete mixed multinomial logit model. By considering a mixed logit model that includes individual-specific variables in the utility specification, our pricing problem reflects well the discrete choice models used in practice. To solve this pricing problem, we design an efficient iterative optimization algorithm that asymptotically converges to the optimal solution. To this end, a linear optimization (LO) problem is formulated, based on the trust-region approach, to find a "good" feasible solution and approximate the problem from below. Another LO problem is designed using piecewise linear relaxations to approximate the optimization problem from above. Then, we develop a new branching method to tighten the optimality gap. The effectiveness of our algorithm is demonstrated on a parking services pricing case, and a benchmark against solvers and existing contributions in the literature are performed.

==> Headlines.tex <==
%%%%%%%%%%%%%%%%%%%%
%PACKAGES
%%%%%%%%%%%%%%%%%%%%

\usepackage[T1]{fontenc}
%\usepackage[latin9]{inputenc}
\usepackage{epsfig}

%\usepackage[left=3cm, right=3cm, top=3cm, bottom=3cm]{geometry}
%\renewcommand{\baselinestretch}{1.25}

\usepackage[english]{babel}

\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{pifont}% http://ctan.org/pkg/pifont

\usepackage{euler,beton}

% Algorithms
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{lineno}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\usepackage{enumerate}
\usepackage{enumitem}

\usepackage[table]{xcolor}% http://ctan.org/pkg/xcolor\usepackage{graphics}
\usepackage{graphicx} %To include figures
\usepackage{adjustbox}
\usepackage{pgfgantt} %Gantt chart
\usepackage{lscape} %Landscape mode for pages
%\usepackage{pdflscape} %Landscape mode for pages in pdf

\usepackage{caption}
\usepackage{subcaption}
\usepackage{comment}

\usepackage{multirow}
\usepackage{booktabs}

\usepackage{appendix}
\usepackage{float}
%\usepackage{color,soul} %Highlight and color
%\usepackage{xcolor}
\usepackage{siunitx}

\usepackage{url}
\usepackage{hyperref}
\hypersetup{colorlinks=true,linkcolor=black,citecolor=black,filecolor=black,urlcolor=black,pdfpagelayout=SinglePage}

% Tikz
\usepackage{tikz}
\usetikzlibrary{plotmarks}
\usetikzlibrary{arrows}

% Bibliography
%\usepackage[dcucite,abbr]{harvard}
%\harvardparenthesis{none}
%\harvardyearparenthesis{round}
\usepackage[comma,authoryear]{natbib}
\bibliographystyle{apalike}
%\usepackage[round]{natbib}
%\bibliographystyle{abbrvnat}


%%%%%%%%%%%%%%%%%%%%
%NEW COMMANDS
%%%%%%%%%%%%%%%%%%%%

\newcommand{\xmark}{\Large\ding{53}}%
\newcommand{\sxmark}{\ding{53}}%
\newcommand{\dingcheck}{\ding{51}}

%\newcommand{\red}[1]{{\color{red} #1}}
%\newcommand{\gray}[1]{{\color{gray} #1}}

\newcommand{\footnoteremember}[2]{
\footnote{#2}
  \newcounter{#1}
  \setcounter{#1}{\value{footnote}}
}
\newcommand{\footnoterecall}[1]{
\footnotemark[\value{#1}]
}

\setlength{\parindent}{0pt}

\sisetup{output-exponent-marker=\ensuremath{\mathrm{e}}}

%%%%%%%%%%%%%%%%%%%%
%COLORS
%%%%%%%%%%%%%%%%%%%%
\definecolor{kellygreen}{rgb}{0.3,0.73,0.09}
\definecolor{lightgreen}{rgb}{0.56,0.93,0.56}
\definecolor{lightyellow}{rgb}{0.94,0.91,0.57}
\definecolor{lightorange}{rgb}{1.0,0.85,0.69}
\definecolor{lightsalmon}{rgb}{1.0,0.63,0.48}
\definecolor{lightcoral}{rgb}{0.94,0.5,0.5}







%%%%%%%%%%%%%%%%%%%%
%HYPHENATION
%%%%%%%%%%%%%%%%%%%%
\hyphenation{models}
\hyphenation{demand}
\hyphenation{analyze}
\hyphenation{utility}
\hyphenation{equili-brium}
\hyphenation{proper-ties}
\hyphenation{know-ledge}
\hyphenation{mo-delled}
\hyphenation{opera-tors}
\hyphenation{compe-titors}
\hyphenation{custo-mers}
\hyphenation{rela-tive}
\hyphenation{indivi-duals}
\hyphenation{condi-tions}
\hyphenation{para-meter}
